Ubiquitous Metadata: Design and Fabrication of Embedded Markers for Real-World Object Identification and Interaction

The convergence of the physical and digital realms has ushered in a new era of immersive experiences and seamless interactions. As the boundaries between the real world and virtual environments blur and result in a "mixed reality," there arises a need for robust and efficient methods to connect physical objects with their virtual counterparts. In this thesis, we present a novel approach to bridging this gap through the design, fabrication, and detection of embedded machine-readable markers. We categorize the proposed marking approaches into three distinct categories: natural markers, structural markers, and internal markers. Natural markers, such as those used in SensiCut, are inherent fingerprints of objects repurposed as machine-readable identifiers, while structural markers, such as StructCode and G-ID, leverage the structural artifacts in objects that emerge during the fabrication process itself. Internal markers, such as InfraredTag and BrightMarker, are embedded inside fabricated objects using specialized materials. Leveraging a combination of methods from computer vision, machine learning, computational imaging, and material science, the presented approaches offer robust and versatile solutions for object identification, tracking, and interaction. These markers, seamlessly integrated into real-world objects, effectively communicate an object's identity, origin, function, and interaction, functioning as gateways to "ubiquitous metadata" - a concept where metadata is embedded into physical objects, similar to metadata in digital files. Across the different chapters, we demonstrate the applications of the presented methods in diverse domains, including product design, manufacturing, retail, logistics, education, entertainment, security, and sustainability.

==> READMEs/README_bibliography.tex <==
%% This file gives an overview on what you will need to do to create a
%% bibliographic database for references, as well as create the actual
%% bibliography for your thesis.

%% You should not need to touch the file biblio.tex.  This merely tells
%% latex to look for the file with the bibliographic info.  The file you
%% want to edit is main.bib.  For each entry, use the appropriate style
%% as designated in the file.

%% Citing your references:

%% When you cite a reference, you need to use the ``key'' you declare in
%% main.bib for the entry.  No one ever sees the keys, but you'll want to
%% use something you will easily remember.  For instance, if you had an
%% entry with:

%% 	   key=geer1

%% Then you would use \cite{geer1} to reference it within your thesis.

%% NOTE: You can not include references in your bibliography that are
%% never cited in your paper by default. If you need to do this, create a
%% key for the entry and at the end of your thesis include the line:

%% \nocite{key}

%% This should be done for every entry which is not explicitly cited.



==> READMEs/README_main.tex <==
%% This file explains the options available to you for editing the file
%% main.tex.

%% The commands in this file allow you to specify options such as
%% spacing, double-sided printing, a draft copy, etc.   By default, 12pt
%% and lgrind are included; lgrind is the 2e style for including code in
%% your thesis.

%% \documentclass[12pt]{mitthesis}
%% \usepackage{lgrind}
%% \pagestyle{plain}

%% You can add options in the documentclass line as follows:

%% 	o  singlespace
%% 	\documentclass[12pt,singlespace]{mitthesis}
	
%% 	o  twoside
%% 	\documentclass[12pt,twoside]{mitthesis}

%% 	o  draft   (make sure to change the pagestyle to drafthead as well)
%% 	\documentclass[12pt,draft]{mitthesis}
%% 	\usepackage{lgrind}
%% 	\pagestyle{drafthead}

%% 	o vi   (for course vi and course viii theses)
%% 	\documentclass[12pt,vi]{mitthesis}

%% Any options you would use for report.sty will work here as well.


%% You should not need to change the first three lines and last two lines
%% below.  Be sure to include an \include command for each file you are
%% including in your thesis.
  
%% \include{cover}
%% \pagestyle{plain}
%% \include{contents}
%% \include{chap1}
%% \include{chap2}
%% \appendix
%% \include{appa}
%% \include{appb}
%% \include{biblio}
%% \end{document}

%% Comment: to include appendices use a single \appendix command followed 
%% by a number of \include{} commands as many files as needed, each of 
%% which should contain a \chapter{} command for the appendix title.


==> READMEs/README_text.tex <==
%% This file includes the basic commands you will need to use within each
%% chapter of your thesis.

%% The file chap1.tex is a sample first chapter.  To get started, you may
%% just want to replace the text and commands in that file as needed.  In
%% general though, for each new chapter you want to do the following:

%% 	o Make sure the name has the extension .tex .  Otherwise, you
%% 	can call it anything you want.  For ease of use, all the
%% 	examples use chap1, chap2, etc.

%% 	o Add a line to the file main.tex that reads:
%% 	\include{yourfilename}

%% 	This should not include the .tex extension, because latex
%% 	assumes that is there.

%% Basic syntax:

%% 	o The first line of each chapter should be:
%% 	\chapter{Chapter Title}

%% 	o To start a new section (labeled chap#.sec# -- as in 1.1,
%% 	1.2, etc):
%% 	\section{Section Heading}

%% 	You can also include subsections:
%% 	\subsection{Heading}




==> appa.tex <==
\chapter{Links}

\begin{itemize}
    \item Code for data generation: \href{https://github.com/HCIELab/InfraTags/tree/main/opencv}{\nolinkurl{https://github.com/HCIELab/InfraTags/tree/main/opencv}}
    
    \item Code for data augmentation and machine learning module: \href{https://github.com/HCIELab/InfraTags/tree/main/ml}{\nolinkurl{https://github.com/HCIELab/InfraTags/tree/main/ml}}
\end{itemize}

\clearpage
\newpage


==> appb.tex <==
\chapter{Figures}

\vspace*{-3in}

\begin{figure}
\vspace{2.4in}
\caption{Armadillo slaying lawyer.}
\label{arm:fig1}
\end{figure}
\clearpage
\newpage

\begin{figure}
\vspace{2.4in}
\caption{Armadillo eradicating national debt.}
\label{arm:fig2}
\end{figure}
\clearpage
\newpage


==> chap6.tex <==
\chapter{Discussion}
\label{thesis-Discussion}

\section{Limitations}
\subsection{Proof of Generalizability}
Our work has shown that the trained model possesses a certain degree of generalizability as it was able to detect InfraredTag codes that were not included in the training set regardless of position, size, orientation, brightness, contrast, and other parameters. The model should work well as long as the original IR image is of sufficient quality. However, the universe of QR codes is infinite. It would not be possible to prove that all QR codes could be universally detected by the model efficiently. Nevertheless, we could add more codes into the validation set and the test set to further improve generalizability. Certain applications in which there is a limited set of possible codes are guaranteed to work efficiently. 

\subsection{The Size and Resolution of InfraredTags}
To speed up processing time, we decided to lower the resolution of the images, which may be problematic if the original resolution of the code is already low. Codes that are too far away from the camera or that are printed on too small an area would appear unresolved and hence may not be detectable. Codes with a lot of fine details, such as dense QR codes, may also suffer because IR imaging is not optimal for capturing fine details with high resolution. Such details might appear as a blurred blob that could not be interpreted.

\subsection{Ground Truth of Fiducial Markers}
Unlike QR codes or other types of codes that only embed information, fiducial markers, such as an ArUco code, can also be used for camera pose estimation. A fiducial marker detector not only identifies the ID of the marker but also computes the 3D distance and 3D orientation of the marker relative to the camera. Distance and orientation are useful for many applications. For example, in driving games, one could use an ArUco code printed on the steering wheel controller to determine whether the player is turning left or right (by measuring the change in the orientation of the code as the player turns the controller). 

There are two "ground truths" for distance and orientation: that in the physical world and that decoded from the marker. One could obtain real-world distance and orientation by making physical measurements, such as by using a measuring tape and a protractor, but this is almost never practical in most settings. It would be more pragmatic to decode distance and orientation from a fiducial marker, but even this approach suffers from certain limitations. As our work has illustrated, the fiducial marker is heavily preprocessed into a binary image before getting decoded. As shown in the second row of Figure \ref{fig:ar_output}, the shape of the processed code is not identical to its real shape. The edges of the code tend to become slightly concave, and this deformity might cause minor errors in the decoded 3D distance and 3D orientation of the marker. Even if we have an equipment that can record an IR video and a normal video simultaneously, it will still be impossible to correct for all those deformities as InfraredTags are invisible to visible light. 

In conclusion, our model can be used, but is not optimized, for determining distances and orientations from fiducial markers. Our model is more suited for applications that do not need such information to be absolutely precise, where a slight error can be tolerated.

\section{Future Work}
\subsection{Other Types of Codes}
For this project, we focused on QR codes and ArUco codes, but InfraredTags can embed any 1D and 2D codes. There are multiple types of codes available beyond the two that we focused on. Among these, many types of 1D barcodes and 2D codes, such as a data matrix and a Maxicode, can be detected by Dynamsoft Barcode Reader \cite{codes}. We expect that the U-Net architecture can work well on other types of codes as well, thereby expanding the varieties of InfraredTag's applications.

\subsection{Augmented Reality: Head-mounted Display}
As mentioned in Chapter 1, imperceptible tags embedded on 3D objects have recently shown promising utility in augmented and virtual reality interactions. One of the devices that tackles augmented and virtual reality is the \textit{HoloLens}\cite{hololens1, hololens2}, a head-mounted display developed by Microsoft. The HoloLens contains multiple cameras, including an IR camera, and provides an infrared light source. Both of these features make the HoloLens compatible with reading InfraredTags. There are varieties of 2D and 3D applications based on QR code and ArUco code detection that can be developed for the HoloLens. For example, the HoloLens can interact with devices and home appliances that have InfraredTags embedded. Scanning InfraredTags on these devices brings up a device control, which the user can manipulate through hand gesture or voice command. The application is illustrated in Figure \ref{fig:app}; even though this figure shows the application on a mobile phone, the application can also be implemented for the HoloLens. Additionally, we can have a fiducial marker embedded on a physical 3D model via InfraredTags. Scanning the fiducial marker brings up a virtual 3D model in the HoloLens. Since the HoloLens is tracking the fiducial marker, the translation and rotation of a physical 3D model also reflects on the virtual 3D model generated in the HoloLens.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{app.png}
    \caption{Controlling appliances using AR application. The user scans a QR code embedded as an InfraredTag on (a) the home speaker to adjust its volume, and (b) the thermostat to adjust the temperature. (c) Pairing a phone with a WiFi router, whose SSID is visible from all sides but the password is visible only from its bottom.}
    \label{fig:app}
\end{figure}

\subsection{Real-time Tangible Interactions}

A fiducial marker can be embedded as an InfraredTag. Since a fiducial marker can be used to track the movement and orientation of an object on which the fiducial marker is embedded, the object can be used as a handheld controller for real-time applications such as video games. Figure \ref{fig:wheel} shows an Infraredtag-embedded 3D printed wheel being wielded as a game controller. The wheel has an ArUco marker InfraredTag embedded. Even though the wheel is rotationally symmetric, the infrared camera can spot the ArUco marker on the wheel, thereby inferring the wheel’s position and orientation relative to the camera. With InfraredTag technology, the handheld controller does not require any electronics as opposed to other approaches \cite{fold}. 
Even though the figure shows the user facing the screen with a camera behind it, the application can also be implemented for a head-mounted display by employing any object with a fiducial marker embedded via InfraredTag as a controller. 

\begin{figure}
    \centering
    \includegraphics[width=0.7\textwidth]{wheel.png}
    \caption{(a) Using the InfraredTag-embedded wheel as a game controller. (b) The ArUco marker embedded on the 3D printed wheel, which contains no electronics components, is invisible under visible light. (c) The ArUco marker embedded on the wheel is only visible to an infrared camera.}
    \label{fig:wheel}
\end{figure}

\subsection{Detection of Markers on Non-rigid Objects}
Recently, a technique to produce tulle-like fabrics from PLA filaments using a fused deposition modeling (FDM) printer has been invented \cite{fabric}.
The technique allows an FDM printer to print thin and flexible textiles.
Objects that can be printed with such a technique are clothes, lamp shades, badminton shuttlecocks, etc. Since InfraredTags are also made of PLA filaments using an FDM printer, InfraredTags can be printed on these objects as well.
This expands the scope of applications to which InfraredTags can contribute. For example, fiducial markers, which are invisible to the naked eye, can be printed on clothes that a person wears. In the future, we plan to use these fiducial markers for motion tracking of the person’s body with a single IR camera. One important challenge regarding this type of tracking is the textiles’ non-rigidity, i.e., the movement of the textile can obscure the markers, thereby making the detection of the markers more challenging. Future work can investigate different data augmentation methods to make the detection model more robust to such occlusion cases.

==> chap7.tex <==
\chapter{Conclusion}
\label{thesis-Conclusion}

InfraredTags have emerged as important tools for tagging objects unobtrusively, with many applications ranging from embedding metadata on grocery items to interacting with a smart device through augmented reality. However, current methods for detecting InfraredTags are relatively slow, partly limiting their use in many settings. A new method for detecting InfraredTags in real time remains an unmet need. In this paper, we sought to devise a new robust method based on machine learning to enable and improve the detection of InfraredTags IR images in real time. We accomplished this by training a U-Net architecture model on a large collection of InfraredTag images as well as augmented InfraredTag images to increase data diversity. The resulting model performed excellently at detecting InfraredTags IR images regardless of the tag's position, size, orientation, brightness, contrast, and other parameters. We decreased the average time per detection from several seconds to 178 ms for QR code detection and 30 ms for ArUco code detection. With detection times reduced to hundreds of milliseconds or below, we believe our model has overcome the existing limitation and effectively permits the use of InfraredTags for real-time applications.

==> old-chap3.tex <==
\chapter{Background}
\section{IR Images}

Unlike images taken with visible light, images taken with infrared can have normal or inverse contrast depending on placement of the light source, the object, and the camera. If the camera and the light source are on the opposite side of the object, infrared from the light source will hit the object, bounce off, and return to the camera. The bright area of a QR code, which reflects infrared, will appear bright, whereas the dark area of the QR code will appear dark. On the contrary, if the camera and the light source are on the same side of the object, there is no reflection of the infrared into the camera. Instead, the signal comes from infrared transmitted from the QR code. The bright area of the QR code, which transmits infrared poorly, will appear dark, whereas the dark area of a QR code, which transmits infrared well, will appear bright. In other words, the image appears as normal contrast if the camera and the light source are on the opposite side of the object but as inverse contrast if the camera and the light source are on the same side of the object. To ensure that our trained model are generalizable, the dataset must include both types of images (light source placements) for each InfraredTag marker.

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{ori_ir.png}
    \includegraphics[width=0.45\textwidth]{invert_ir.png}
    \caption{The IR image taken with a light source and a camera on the opposite side of the object (left). The IR image taken with a light source and a camera on the same side of the object (right).}
    \label{fig:ir_image}
\end{figure}

\section{Image Processing Techniques}
\subsection{CLAHE}

Adaptive histogram equalization is an image-processing technique used for improving the contrast of an image. However, it could also inadvertently lead to overamplification of noise in the image. Contrast limited adaptive histogram equalization (CLAHE) is a variant of this technique that obviates this side effect by limiting contrast amplification. In a typical CLAHE process, the image is first split into tiles, and CLAHE is performed individually on each tile. In each tile, the pixels' intensities in the range $[0,255]$ are plotted into a histogram. CLAHE limits contrast amplification by setting a clipLimit. For each intensity, the frequency will be clipped to a clipLimit. Any amount exceeding clipLimit will be cumulated and redistributed equally among all intensities. Then a probability density function (PDF) and a cumulative distribution function (CDF) of the histogram are calculated, respectively. Afterwards, the intensity $x$ of the pixel will be reassigned as

\[x = \text{CDF}(x) \cdot 255\]

\subsection{Gaussian Blur}

A Gaussian blur, or Gaussian smoothing, is the process that blurs an image with a Gaussian function:

\[G(x,y) = \frac{1}{2\pi\sigma^{2}}e^{-\frac{x^2+y^2}{2\sigma^2}}\]

where $x$ is the distance from the origin in the horizontal axis, $y$ is the distance from the origin in the vertical axis, and $\sigma$ is the standard deviation of the Gaussian distribution.

Applying a Gaussian blur to an image is the same as convolving an image. Hence, in the blurred image, each pixel will be the weighted average of its neighbor pixels in the original image. The size of the kernel for convolution is one of the parameters of a Gaussian blur. Applying a Gaussian blur also reduces the high-frequency components in an image; thus, a Gaussian blur is a low-pass filter.

\subsection{Gaussian Adaptive Thresholding}

Thresholding is the method that is used to turn a grayscale image to a binary image. Applying a simple thresholding with a threshold $T$ on an image $I$ gives an output image $O$ where

\[ O_{ij} = 
    \begin{cases} 
      255 & \text{if } I_{ij} \geq T, \\
      0 & \text{otherwise},
   \end{cases}
\]

$I_{ij}$ is the value of pixel $(i,j)$ of the input image $I$, and $O_{ij}$ is the value of pixel $(i,j)$ of the output image $O$. This thresholding method is simple but might break down under unfavorable lighting conditions, such as when there is a shadow or a glare in the image, which could be falsely categorized as dark and bright pixels, respectively. Such lighting conditions often have a localized effect, suggesting that this problem can be solved by having a different threshold for different locations within the image. Adaptive thresholding, a thresholding method where the threshold is dynamically changed over the image, is used. One variant of adaptive thresholding is Gaussian adaptive thresholding. Calculating the threshold of each pixel is the same as convolving the image. Hence, the threshold of each pixel is the weighted average of its neighboring pixels, and the weight is calculated using a Gaussian function in the same manner as calculation of a Gaussian blur. The size of the kernel for convolution is one of the parameters of Gaussian adaptive thresholding.


==> signature.tex <==
% -*- Mode:TeX -*-
%
% Some departments (e.g. Chemistry) require an additional cover page
% with signatures of the thesis committee.  Please check with your
% thesis advisor or other appropriate person to determine if such a 
% page is required for your thesis.  
%
% If you choose not to use the "titlepage" environment, a \newpage
% commands, and several \vspace{\fill} commands may be necessary to
% achieve the required spacing.  The \signature command is defined in
% the "mitthesis" class
%
% The following sample appears courtesy of Ben Kaduk <kaduk@mit.edu> and
% was used in his June 2012 doctoral thesis in Chemistry. 

\begin{titlepage}
\begin{large}
This doctoral thesis has been examined by a Committee of the Department
of Chemistry as follows:

\signature{Professor Jianshu Cao}{Chairman, Thesis Committee \\
   Professor of Chemistry}

\signature{Professor Troy Van Voorhis}{Thesis Supervisor \\
   Associate Professor of Chemistry}

\signature{Professor Robert W. Field}{Member, Thesis Committee \\
   Haslam and Dewey Professor of Chemistry}
\end{large}
\end{titlepage}


